Knowledge-Augmented Reasoning Distillation for Small Language Models in Knowledge-Intensive Tasks

Large Language Models (LLMs) have shown promising performance in knowledge-intensive reasoning tasks that require a compound understanding of knowledge. However, deployment of the LLMs in real-world applications can be challenging due to their high computational requirements and concerns on data privacy. Previous studies have focused on building task-specific small Language Models (LMs) by fine-tuning them with labeled data or distilling LLMs. However, these approaches are ill-suited for knowledge-intensive reasoning tasks due to the limited capacity of small LMs in memorizing the knowledge required. Motivated by our theoretical analysis on memorization, we propose Knowledge-Augmented Reasoning Distillation (KARD), a novel method that fine-tunes small LMs to generate rationales obtained from LLMs with augmented knowledge retrieved from an external knowledge base. Moreover, we further propose a neural reranker to obtain documents relevant to rationale generation. We empirically show that KARD significantly improves the performance of small T5 and GPT models on the challenging knowledge-intensive reasoning datasets, namely MedQA-USMLE, StrategyQA, and OpenbookQA. Notably, our method makes the 250M T5 models achieve superior performance against the fine-tuned 3B models, having 12 times larger parameters, on both MedQA-USMLE and StrategyQA benchmarks.

==> texts/11_app_theory.tex <==
\allowdisplaybreaks

\section{Motivation: Effect of Knowledge-Augmentation on Memorization} \label{app:theory}

\subsection{Additional Details and Discussion}

 We adopted the abstracted language problem, i.e., the next-symbol prediction problem with reference strings $c_j \sim \mathrm{Uniform}\left(\{0,1\}^d\right)$, considered in the main text of \citep{brown2021memorization} with no symbol corruption. In this  problem,  the random process $P \sim q$ is defined by drawing $c_j\in\{0,1\}^d$ uniformly at random as  $c_j \sim \mathrm{Uniform}\left(\{0,1\}^d\right)$ for all $j\in [N]$: a set $\{c_j\}_{j=1}^N$ corresponds to a $P$. Then,  the random process $(Z,Y) \sim P$ is defined by sampling $j\sim \mathrm{Uniform}\left([N]\right)$ and  $\ell\sim \mathrm{Uniform}\left(\{0,1,2,\dots,d-1\}\right)$ and by setting $Z=(j ,c_j(1:\ell))$ and $Y=c_j(\ell+1)$, where $c_j(1:l)$ denotes the first $l$ symbols of $c_j$ and $c_j(l+1)$ is $(l+1)$-th symbol of $c_j$. The training data $X\sim P^{\otimes n}$ contains $((Z_i,Y_i))_{i=1}^n$  generated by the same process $n$ times independently.

Recall  that the inference algorithm $\varphi$ uses a KB denoted by $S$ such that $|S|=N+R$ and $\{c_j\}_{j=1}^N \subseteq S$. Here, $S$ is a set and \textit{not} ordered; therefore we do not know the identifier $j$ of each $s\in S$ and which $s \in S$ is useful given each $(Z,Y)$. Thus, this still requires learning and memorizing some information from the training data $X$. 

In Theorem \ref{thm:2}, $N$ (or $R$) is  the number of useful (or unuseful) documents in KB to be  extracted by a retriever. Thus,   $N+R$ is the total number of possible documents to be retrieved. As $N+R$ increases, we need to memorize more information of the training data to get the best match at test time. Theorem \ref{thm:2} shows that this increase happens only in the log rate,   $\log_2(N+R)$. Thus, we can get improvements when the size of   KB ($d$) is larger than \textit{the log} of the number of possible choices to be retrieved by the retriever ($\log_2(N+R)$). 

Moreover, unlike Theorem \ref{thm:1}, we can remove the dependence on $n$   and have  $I(X; \Acal(X)|P)=O(N\log_2(N+R))$  in Theorem \ref{thm:2} when the training size $n$ grows at a faster rate than the number of the useful documents  $N$. This is because our proof does not rely on the high probability of having a singleton training sample per each reference $c_j$ unlike the proof of   \citep{brown2021memorization}.  

\subsection{Proof of Theorem \ref{thm:2}}
\begin{proof}
Let $\epsilon>0$ and  $m=\log_2((1-(\frac{N-1}{N})^n) \frac{(N+R)^2 - (N+R)}{2\epsilon})$. Since the distribution over subpopulation is uniform, \begin{align*}
\errKB(\Acal) = \sum_{j=1}^N\Pr(Q_{j})\Pr_{\substack{}}(E_{0}|Q_{j})=\frac{1}{N}\sum_{j=1}^N\Pr_{\substack{}}(E_{0}|Q_{j}),
\end{align*}
where  $E_{0}$ is the event of $\varphi(Z,\Acal(X),S)\neq Y$ and $Q_j$ is the event that the subpopulation of the test sample $(Z,Y) \sim P$ is $j$.  Let  $E_{1}^j$ be the event of having at least one training data sample ($(Z_i, Y_i) \in X$) in the subpopulation $j$ of the test sample $(Z,Y) \sim P$. 
Then,
\begin{align*}
\Pr_{\substack{}}(E_{0}| Q_j)=\Pr(E_{1}^{j}|Q_j)\Pr_{\substack{}}(E_{0}| Q_j,E_{1}^{j})+\Pr(\bE_{1}^{j}|Q_j)\Pr_{\substack{}}(E_{0}| Q_j,\bE_{1}^{j})
\end{align*}
where $\bar E_1^j$ is the complement of $E_1^j$. Denote by $\ell_x^{j}$ the length of training sample, and by $\ell_t^{j}$ the length of the test sample,  in the subpopulation $j$. 
Let
$E_{2}^j$ be the event of  $\ell_{x}^j \ge m$ for at least one training sample in the subpopulation $j$, and $E_{3}^j$ be the event of $\ell_t^j< \ell_x^j$ for at least one training sample  in the subpopulation $j$. Then, 
\begin{align*}
\errKB(\Acal) =&\frac{1}{N}\sum_{j=1}^N\Pr(E_{1}^{j}|Q_j)\Pr(E_{2}^{j}|Q_j,E_{1}^{j})\Pr_{\substack{}}(E_{0}| Q_j,E_{1}^{j},E_{2}^{j})
\\ & + \frac{1}{N}\sum_{j=1}^N\Pr(E_{1}^{j}|Q_j)\Pr(\bE_{2}^{j}|Q_j,E_{1}^{j})\Pr(E_{3}^{j}|Q_j,E_{1}^{j},\bE_{2}^{j})\Pr_{\substack{}}(E_{0}| Q_j,E_{1}^{j},\bE_{2}^{j},E_{3}^{j})
\\ & + \frac{1}{N}\sum_{j=1}^N\Pr(E_{1}^{j}|Q_j)\Pr(\bE_{2}^{j}|Q_j,E_{1}^{j})\Pr(\bE_{3}^{j}|Q_j,E_{1}^{j},\bE_{2}^{j})\Pr_{\substack{}}(E_{0}| Q_j,E_{1}^{j},\bE_{2}^{j},\bE_{3}^{j})
\\ & +\frac{1}{N}\sum_{j=1}^N\Pr(\bE_{1}^{j}|Q_j)\Pr_{\substack{}}(E_{0}| Q_j,\bE_{1}^{j}).
\end{align*}
Define $E_{0}^*$ to be  the event of $M_{\mathrm{OPT}}(Z)\neq Y$ where $M_{\mathrm{OPT}}=\AcalO(X)$. Then, the same decomposition holds for $\err(\AcalO)$ yielding that 
\begin{align*}
\err(\AcalO)=&\frac{1}{N}\sum_{j=1}^N\Pr(E_{1}^{j}|Q_j)\Pr(E_{2}^{j}|Q_j,E_{1}^{j})\Pr_{\substack{}}(E_{0}^{*}| Q_j,E_{1}^{j},E_{2}^{j})
\\ & + \frac{1}{N}\sum_{j=1}^N\Pr(E_{1}^{j}|Q_j)\Pr(\bE_{2}^{j}|Q_j,E_{1}^{j})\Pr(E_{3}^{j}|Q_j,E_{1}^{j},\bE_{2}^{j})\Pr_{\substack{}}(E_{0}^{*}| Q_j,E_{1}^{j},\bE_{2}^{j},E_{3}^{j})
\\ & + \frac{1}{N}\sum_{j=1}^N\Pr(E_{1}^{j}|Q_j)\Pr(\bE_{2}^{j}|Q_j,E_{1}^{j})\Pr(\bE_{3}^{j}|Q_j,E_{1}^{j},\bE_{2}^{j})\Pr_{\substack{}}(E_{0}^{*}| Q_j,E_{1}^{j},\bE_{2}^{j},\bE_{3}^{j})
\\ & +\frac{1}{N}\sum_{j=1}^N\Pr(\bE_{1}^{j}|Q_j)\Pr_{\substack{}}(E_{0}^{*}| Q_j,\bE_{1}^{j}).
\end{align*}
Since the probabilities are non-negative,  by ignoring some terms, we have that
\begin{align*}
\err(\AcalO) \ge & \frac{1}{N}\sum_{j=1}^{N}\Pr(\bE_{1}^{j}|Q_j)\Pr(E_{0}^{*}| Q_j,\bE_{1}^{j})
\\ & +\frac{1}{N}\sum_{j=1}^{N}   \Pr(E_{1}^{j}|Q_j)\Pr(\bE_{2}^{j}|Q_j,E_{1}^{j})\Pr(\bE_{3}^{j}|Q_j,E_{1}^{j},\bE_{2}^{j})\Pr_{\substack{}}(E_{0}^{*}| Q_j,E_{1}^{j},\bE_{2}^{j},\bE_{3}^{j}).
\end{align*}
 Since these two terms $\Pr(E_{0}^{*}| Q_j,\bE_{1}^{j})$ and $\Pr_{\substack{}}(E_{0}^{*}| Q_j,E_{1}^{j},\bE_{2}^{j},\bE_{3}^{j})$ correspond to the errors when the test data comes into the place with no information from the training data, the memorizing data does not help and the random guess achieves the best performance. Moreover, these two cases can be detected at test time by  $(\varphi, \Acal)$ by memorizing  the first $\min(m,\ell_{x}^j)$ bits of an input sequence in the training data $X$ and $j$ (i.e., $\min(m,\ell_{x}^j)+1$ bits in total) for at most one training sample per $j \in[N]$. Thus, we choose $\Acal$ to memorize the first $\min(m,\ell_{x}^j)$ bits and $j$  for at most one training sample per $j \in[N]$; i.e., we memorize $\min(m,\ell_{x}^j)+1\le m+1$ bits for at most $\min(N,n)$ training samples. In total, we memorise at most $\min(N,n)(m+1)$ bits.  Then, these two terms are the same for $\err(\AcalO)$ and $\errKB(\Acal)$ by detecting these cases (with  memorization) and generating a random guess for these cases. Thus, \begin{align*}
\err(\AcalO) \ge & \frac{1}{N}\sum_{j=1}^{N}\Pr(\bE_{1}^{j}|Q_j)\Pr(E_{0}^{}| Q_j,\bE_{1}^{j})
\\ & +\frac{1}{N}\sum_{j=1}^{N}   \Pr(E_{1}^{j}|Q_j)\Pr(\bE_{2}^{j}|Q_j,E_{1}^{j})\Pr(\bE_{3}^{j}|Q_j,E_{1}^{j},\bE_{2}^{j})\Pr_{\substack{}}(E_{0}^{}| Q_j,E_{1}^{j},\bE_{2}^{j},\bE_{3}^{j}).
\end{align*}
Therefore,  
\begin{align*}
&\errKB(\Acal) -\err(\AcalO) 
\\ & \le \frac{1}{N}\sum_{j=1}^N\Pr(E_{1}^{j}|Q_j)\Pr(E_{2}^{j}|Q_j,E_{1}^{j})\Pr_{\substack{}}(E_{0}| Q_j,E_{1}^{j},E_{2}^{j})
\\  & \quad+ \frac{1}{N}\sum_{j=1}^N\Pr(E_{1}^{j}|Q_j)\Pr(\bE_{2}^{j}|Q_j,E_{1}^{j})\Pr(E_{3}^{j}|Q_j,E_{1}^{j},\bE_{2}^{j})\Pr_{\substack{}}(E_{0}| Q_j,E_{1}^{j},\bE_{2}^{j},E_{3}^{j})
\\ & \quad + \frac{1}{N}\sum_{j=1}^N\Pr(E_{1}^{j}|Q_j)\Pr(\bE_{2}^{j}|Q_j,E_{1}^{j})\Pr(\bE_{3}^{j}|Q_j,E_{1}^{j},\bE_{2}^{j})\Pr_{\substack{}}(E_{0}| Q_j,E_{1}^{j},\bE_{2}^{j},\bE_{3}^{j})
\\ & \quad+\frac{1}{N}\sum_{j=1}^N\Pr(\bE_{1}^{j}|Q_j)\Pr_{\substack{}}(E_{0}| Q_j,\bE_{1}^{j}) - \frac{1}{N}\sum_{j=1}^{N}\Pr(\bE_{1}^{j}|Q_j)\Pr(E_{0}^{}| Q_j,\bE_{1}^{j})
\\ & \quad  -\frac{1}{N}\sum_{j=1}^{N}   \Pr(E_{1}^{j}|Q_j)\Pr(\bE_{2}^{j}|Q_j,E_{1}^{j})\Pr(\bE_{3}^{j}|Q_j,E_{1}^{j},\bE_{2}^{j})\Pr_{\substack{}}(E_{0}^{}| Q_j,E_{1}^{j},\bE_{2}^{j},\bE_{3}^{j}).
\\  = & \frac{1}{N}\sum_{j=1}^N\Pr(E_{1}^{j}|Q_j)\Pr(E_{2}^{j}|Q_j,E_{1}^{j})\Pr_{\substack{}}(E_{0}| Q_j,E_{1}^{j},E_{2}^{j}) 
\\ & +\frac{1}{N}\sum_{j=1}^N  \Pr(E_{1}^{j}|Q_j)\Pr(\bE_{2}^{j}|Q_j,E_{1}^{j})\Pr(E_{3}^{j}|Q_j,E_{1}^{j},\bE_{2}^{j})\Pr_{\substack{}}(E_{0}| Q_j,E_{1}^{j},\bE_{2}^{j},E_{3}^{j})
\end{align*}
Here, we notice that $\Pr_{\substack{}}(E_{0}| Q_j,E_{1}^{j},\bE_{2}^{j},E_{3}^{j})=0$ because $\Acal$ memorizes the first $\min(m,\ell_{x}^j)$ bits, where $\min(m,\ell_{x}^j)=\ell_x^j$  conditioned on $\bE_2^{j}$, and because  this is conditioned on the events $E_1^{j}$ and $E_3^{j}$. That is, $\Pr_{\substack{}}(E_{0}| Q_j,E_{1}^j,\bE_{2}^j,E_{3}^j)$ is the error probability when we have a training sample with the length $\ell_x^j$ larger than the test sample length $\ell_t^j$ on the same subpopulation and $\ell_x^j=\min(m,\ell_{x}^j)$ bits of  the training samples are memorized. In this case, we can simply output the next symbol for the test sample from the memorized training sample, yielding  $\Pr_{\substack{}}(E_{0}| Q_j,E_{1}^j,\bE_{2}^j,E_{3}^j)=0$.
Therefore,
\begin{align} \label{eq:1}
\errKB(\Acal) -\err(\AcalO) 
\le \frac{1}{N}\sum_{j=1}^N\Pr(E_{1}^j|Q_j)\Pr(E_{2}^j|Q_j,E_{1}^j)\Pr_{\substack{}}(E_{0}| Q_j,E_{1}^j,E_{2}^j). 
\end{align}  
In the case of the events $Q_j,E_{1}^j$ and $E_{2}^j$, $\Acal(X)$ memorized  $\min(m,\ell_{x}^j)=m$  bits of the input sequence in the training sample for at least one training sample in  the  subpopulation $j$ of the test sample. In this case, at  test time, $\varphi$ first chooses one training sample  in  the  same subpopulation $j$ of the test sample (we can do this because the non-label part $Z$ contains the subpopulation information $j$ in both test sample $(Z,Y) \sim P$ and in the training sample; see \citealt{brown2021memorization}). Then,  $\varphi$   
uses the memorized $m$ bits of this training sample to search $S$; i.e., it picks $s \in S$ such that the first $m$ bits of $s$ matches with the memorized $m$ bits of the training sample. If there are more than one $s \in S$ that satisfies this condition, then it randomly picks one of them. Note that in this case of the events $Q_j,E_{1}$ and $E_{2}$, there is at least one match; there exists $s \in S$ the first $m$ bits of $s$ matches with the memorized $m$ bits of the training sample. 

 Thus, if there is no more than one $s \in S$ that satisfies this condition,
then the inference algorithm $\varphi$ uniquely determines the  reference string $c_j$ of the test sample  $(Z,Y) \sim P$. With  the  reference string $c_j$ of the test sample,  $\varphi$ then predict the next symbol of the test sample by  outputting $(\ell_{t}^j+1)$-th symbol of   the  reference string $c_j$, where  $\ell_{t}^j$ is computable by computing the length of the test input $Z$ without any information of training samples. Therefore, if there is no more than one $s \in S$ that satisfies the above condition, then  $\varphi$  makes a correct prediction. This implies that
if  $s$ and $s'$ do \textit{not} have  the same first $m$ bits for all $s,s' \in S  \text{ with } s\neq s'$, then  $\varphi$  makes a correct prediction.  By taking complement, this means that the error occurs only if there exist $s,s' \in S$ with $s\neq s'$ such that  $s$ and $s'$ have the same first $m$ bits.
Therefore,\begin{align*}
\Pr_{\substack{}}(E_{0}| Q_j,E_{1}^j,E_{2}^j) &\le  \Pr (\exists s,s' \in S  \text{ with } s\neq s' \text{ such that $s$ and $s'$ have the same first $m$ bits})
\\ & =  \Pr(\cup_{\{s,s'\}\in \mathcal{T}}\{ \text{$s$ and $s'$ have the same first $m$ bits}\})
\\ &\leq \sum_{\{s, s^\prime\}\in \Tcal}\Pr(\{\text{$s$ and $s'$ have the same first $m$ bits} \})
\\ & \leq \binom{N+R}{2} \frac{1}{2^m} = \frac{(N+R)^2 - (N+R)}{2}\frac{1}{2^m} 
\end{align*}
where $ \mathcal{T} = \{\{s,s'\} | s,s'\in S, s\neq s'\}$. Since $m=\log_2((1-(\frac{N-1}{N})^n) \frac{(N+R)^2 - (N+R)}{2\epsilon})$, 
\begin{align*} 
\Pr_{\substack{}}(E_{0}| Q_j,E_{1}^j,E_{2}^j) & \le\frac{(N+R)^2 - (N+R)}{2}\frac{1}{(1-(\frac{N-1}{N})^n) \frac{(N+R)^2 - (N+R)}{2\epsilon}} 
\\ & =\frac{}{}\frac{\epsilon}{1-(\frac{N-1}{N})^n}. 
\end{align*}  
Plugging this into \eqref{eq:1},
\begin{align*}
\errKB(\Acal) -\err(\AcalO) \le\frac{1}{N}\sum_{j=1}^N\Pr(E_{1}^j|Q_j)\Pr(E_{2}^j|Q_j,E_{1}^j)\frac{\epsilon}{1-(\frac{N-1}{N})^n}.
\end{align*}
Since $\Pr(E_{2}^j|Q_j,E_{1}^j)\le 1$ and $\Pr(E_{1}^j|Q_j)=1-\Pr(\bE_{1}^j|Q_j^j)=1-(\frac{N-1}{N})^n$,
\begin{align*}
\errKB(\Acal) -\err(\AcalO) \le\frac{1}{N}\sum_{j=1}^N\epsilon = \epsilon.
\end{align*}
Since we only require $m+1$ bits for at most $\min(N,n)$ training samples from the above construction of $\Acal$ and $\varphi$, we have that  $I(X; \Acal(X)|P)=O(\min(N,n)m)$ while achieving $\errKB(\Acal) -\err(\AcalO) \le \epsilon$ for any $\epsilon>0$.   
\end{proof}
